COST Action IC 1402 ArVI: Runtime Verification Beyond Monitoring -- Activity Report of Working Group 1

This report presents the activities of the first working group of the COST Action ArVI, Runtime Verification beyond Monitoring. The report aims to provide an overview of some of the major core aspects involved in Runtime Verification. Runtime Verification is the field of research dedicated to the analysis of system executions. It is often seen as a discipline that studies how a system run satisfies or violates correctness properties. The report exposes a taxonomy of Runtime Verification (RV) presenting the terminology involved with the main concepts of the field. The report also develops the concept of instrumentation, the various ways to instrument systems, and the fundamental role of instrumentation in designing an RV framework. We also discuss how RV interplays with other verification techniques such as model-checking, deductive verification, model learning, testing, and runtime assertion checking. Finally, we propose challenges in monitoring quantitative and statistical data beyond detecting property violation.

==> conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

==> header.tex <==
\title{%
COST Action IC 1402 ArVI: Runtime Verification Beyond Monitoring\\
Report of Working Group 1
% Uncomment the following line if there is some acknowledgment.
%\thanks{The authors would like to gratefully acknowledge.}
}
% In case the submission is double blind
%\author{\vspace{-1em}}
%\institute{\vspace{-1em}}
% In case the subbmision is single blind.
%
\author{
Author 1\inst{1}
\and
Author 2\inst{2}
\and
Author 3\inst{1}
}
\institute{
Univ. Grenoble Alpes, CNRS, Inria, Grenoble INP, LIG, 38000 Grenoble, France
\email{{\{author1,author3\}}@univ-grenoble-alpes.fr}
\and
Another institute.\\
\email{author2@inst2.com}
}
\titlerunning{Short title}
\authorrunning{Author1, Author2, Author3}

==> macros.tex <==
%
%Anottation of the paper by message passing.
%
\newcommand{\yf}[2]{\TODO{YF@#1:\\#2}}
\newcommand{\ck}{\\CHECK \& KILL.}
%
% Generic shorthands
%
%\newcommand{\ie}{\textsl{i.e.,}\xspace}
%\newcommand{\eg}{{e.g.,}\xspace}
%
% Maths
%
%\DeclareMathOperator{\opname}{opname}

